An Experimental Study of Low-Latency Video Streaming over 5G

Low-latency video streaming over 5G has become rapidly popular over the last few years due to its increased usage in hosting virtual events, online education, webinars, and all-hands meetings. Our work aims to address the absence of studies that reveal the real-world behavior of low-latency video streaming. To that end, we provide an experimental methodology and measurements, collected in a US metropolitan area over a commercial 5G network, that correlates application-level QoE and lower-layer metrics on the devices, such as RSRP, RSRQ, handover records, etc., under both static and mobility scenarios. We find that RAN-side information, which is readily available on every cellular device, has the potential to enhance throughput estimation modules of video streaming clients, ultimately making low-latency streaming more resilient against network perturbations and handover events.

==> result_old.tex <==
% \vspace{-0.1in}


\section{Measurement Results and Analysis}
\label{results}

While in the previous section, we specified our experimental setup and detailed the data collection process, in this section we delve into the analysis of our low-latency streaming measurements under the three mobility scenarios considered.
\subsection{QoE Metrics Calculation}
To that end, each playback session is divided into multiple 1-minute runs based on which the following metrics are calculated:

\noindent\textbf{Weighted Bitrate.} We define a new metric called weighted bitrate. For each session of video playback, the player switches between bitrates to adapt to varying network conditions. Depending on how long the player stayed on a particular bitrate, we calculate the weighted bitrate as below:

%Weighted Bitrate = \frac{$\sum_{n=1}^{\infty} 2^{-n}}
%Weighted Bitrate = \frac{b1 (t1-t0) + b2 (t2-t1) + b3(t3-t2)} {t3-t0}
%\ [ Weighted Bitrate =\frac{b1 (t1-t0) + b2 (t2-t1) + b3(t3-t2}{(t3-t0)} \ ] \ \
%\[Weighted Bitrate = \frac{\sigma b_i * \Delta t_i}{\sigma \Delta t_i}\]

\[Weighted Bitrate = \frac{\sum ( b_i * \Delta t_i)}{\sum \Delta t_i}\]

Here $b_i$ is a bitrate and $\Delta$ $t_i$ is the duration of time that the video bitrate remained at $b_i$.
%is the time difference between two consecutive timestamps where the bitrate switch was observed. 

\noindent\textbf{Latency Lag.} For each playback session, we calculate the achieved latency by averaging the per-second data extracted from the ExoPlayer logs. We then subtract the average value from the target value set at the server. This metric denotes the difference between achieved  and target latency.

\noindent\textbf{Bitrate Switch Count.} For each playback session, we count the number of switches in bitrate,  normalized over the playback duration.

\noindent\textbf{Rebuffer Event Count.} For each playback session, we count the number of re-buffering events, normalized over the playback duration.
\begin{figure}[!htbp] 
  \centering
    \begin{subfigure}{.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/ik_static_compare.pdf}
        % \caption{Latency Lag}
        \label{fig:static_latencylag} 
    \end{subfigure}\hspace{0.05\textwidth}
 %    \begin{subfigure}{.35\textwidth}
 %        \centering
 %        \includegraphics[width=0.99\textwidth]{figs/boxplot_wb.pdf}
 %        \caption{Weighted bitrate.}
	% \label{fig:static_wbitrate}
	% \end{subfigure}
\caption{Performance in Static Scenario}
\label{fig:wifi_rates}
\end{figure}


\begin{figure*}[t]
  \centering
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/ik_static_mobility_compare_latency.pdf}
        
        \caption{Latency Lag}
        \label{fig:comp_ld}
	\end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/ik_static_mobility_compare_wb.pdf}
        
        \caption{Weighted Bitrate}
	\label{fig:comp_wb} 
    \end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/ik_static_mobility_compare_nb.pdf}
        \caption{Bitrate Switch Count}
        \label{fig:comp_bsw}
    \end{subfigure}

\caption{Average QoE Metrics over 5G (peak) Under Static and Walking Scenarios}
\label{fig:scenario_compare}
\end{figure*}

\begin{figure*}[t]
  \centering
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/profile_2_scatter.pdf}
        
        \caption{Profile S2-C0.1-L3}
        \label{fig:llrb_2}
	\end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/profile_3_scatter.pdf}
        
        \caption{Profile S3-C0.1-L4}
	\label{fig:llrb_3} 
    \end{subfigure}
    \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/profile_4_scatter.pdf}
        \caption{Profile S4-C0.1-L5}
        \label{fig:llrb_4}
    \end{subfigure}

\caption{Latency Lag as a function of Rebuffer Events}
\label{fig:latency_rebuf_compare}
\end{figure*}

 \begin{figure*}
  \centering
   \begin{subfigure}{0.75\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/sample_walking.pdf}
        \caption{Sample Walking Run}
        \label{fig:sample_walking}
	\end{subfigure}
    \begin{subfigure}{0.75\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/sample_driving.pdf}
        \caption{Sample Driving Run}
	\label{fig:sample_driving} 
    \end{subfigure}
\caption{Mobility Scenario Case Study}
\label{fig:sample_driving_run}
\vspace{-0.1in}
\end{figure*}
%\blue{Describe how to calculate the metrics such as weighted bitrate, etc.}





\subsection{Static Scenario}
We first look at the streaming performance in the static scenario. In Fig. \ref{fig:wifi_rates}, we box-plot the latency lag and weighted bitrate of each profile over the WiFi channel and 5G non-peak and peak hours. As expected, the player's bitrate never switches over WiFi and the weighted bitrate remains at 6 Mbps (the highest possible) for all the runs. The lowest latency lag is observed for profiles with the lowest segment size of 2 s. We notice a negligible difference (i.e., 250 ms for segment size 2 s) in latency lag for the profiles with the same segment size but different chunk sizes (0.1/0.5/1 s). The latency lag also increases with segment size. For example, for the S2-C0.1-L3, profile, the median latency lag observed is 930 ms whereas, for the S3-C0.1-L4 and the S4-C0.1-L5 profiles, the values are 1.59 s and 1.96 s respectively. From this, we conclude that the player achieves the lowest latency lag with the smallest segment size setting.

\begin{table}[ht]
    \centering
    \caption{Weighted Bitrate (Mbps) under static scenario}
    \label{tab:table_wb}
    {\small
    \resizebox{0.8\columnwidth}{!}{\begin{tabular}{|c |c |c |c |}
    \hline
    \textbf{Profile} & \textbf{WiFi} & \textbf{5G (Non-peak)} & \textbf{5G (Peak)}  \\ \hline
     S2-C0.1-L3 & 6 $\pm$ 0 & 5.87 $\pm$ 0.37 & 5.75 $\pm$ 0.47  \\ 
     S2-C0.5-L3 & 6 $\pm$ 0 & 5.88 $\pm$ 0.24 & 5.35 $\pm$ 1.12  \\ 
     S2-C01-L3 & 6 $\pm$ 0 & 5.69 $\pm$ 0.55 & 5.75 $\pm$ 0.75  \\ \hline
     S3-C0.1-L4 & 6 $\pm$ 0 & 5.81 $\pm$ 0.96 & 6 $\pm$ 0 \\ 
     S3-C0.5-L4 & 6 $\pm$ 0 & 5.9 $\pm$ 0.38 & 5.84 $\pm$ 0.47  \\ 
     S3-C1-L4 & 6 $\pm$ 0 & 6 $\pm$ 0 & 5.82 $\pm$ 0.53  \\ \hline
     S4-C01-L5 & 6 $\pm$ 0 & 6 $\pm$ 0 & 5.55 $\pm$ 0.64  \\ 
     S4-C0.5-L5 & 6 $\pm$ 0 & 6 $\pm$ 0 & 5.76 $\pm$ 0.66  \\ 
     S4-C1-L5 & 6 $\pm$ 0 & 6 $\pm$ 0 & 5.86 $\pm$ 0.33  \\ \hline
    \end{tabular}}}
    \vspace{-0.05in}
\end{table}

These findings also hold true for the runs over the 5G network. As expected, from Table \ref{tab:table_wb} we see that the achieved average weighted bitrate is higher and the latency lag is lower over WiFi compared to 5G. For runs over 5G, in general, the average weighted bitrate for non-peak hours is slightly higher than for peak hours. For some profiles, for example, the S2-C1-L3 profile, the average weighted bitrate is slightly lower (5.69 Mbps) for non-peak hours compared to that of peak hours (5.74 Mbps). This has an impact on the latency lag as we see that for peak and non-peak hours, the median values are 1.5 s and 1.7 s respectively. In this case, the player stayed on a higher bitrate at the cost of higher latency. 

From our observations we conclude the following, (1) in general low-latency streaming works over 5G under static conditions, (2) the performance of low-latency streaming depends on the server-side configuration. It is imperative to use a shorter segment size as the achieved end-to-end latency is the lowest however chunk size variation does not have an impact on the performance, and (3) network load does not have a significant impact on the performance of streaming. 


\subsection{Mobility Scenario} In this section, we discuss the results of the two mobility scenarios (i.e., walking and driving) and compare those to the static scenarios. From static scenario results we learned that for each segment size, the profiles (S2-C0.1-L3, S3-C0.1-L4, and S4-C0.1-L5) with the lowest target latency set achieved the best overall performance. For the mobility scenarios, we select these profiles for further evaluation. In Fig. \ref{fig:scenario_compare}, we plot the average QoE metrics gathered over 5G peak hours under static, walking, and driving scenarios. For the S2-C0.1-L3 profile, as expected, the latency lag is found to be lower in static conditions than in the walking scenario but higher compared to driving conditions. If we look at Fig. \ref{fig:comp_wb}, we see that for the same profile, the median weighted bitrate is noticeably higher (mean 6 Mbps) in static scenarios compared to that of walking and driving (median values of 3 and 1 Mbps, respectively). For mobility scenarios, the player bitrate often reduces to lower values while the network conditions change and never switch up due to the conservative configuration of the player. We debugged the player behavior and found that before switching bitrates the player checks if the selected track is of higher quality than the currently selected one, and if so, whether it has a sufficient buffer to safely switch up. If not, it will defer switching up for the time. We noticed that the player has configured the \hyp{"DEFAULT\_MIN\_DURATION\_FOR\_QUALITY\_INCREASE\_MS"} value to be 10 s. In contrast, the average buffer occupancy for low latency streaming is significantly low for example, 1 s average buffer occupancy for 2 s segment size. This causes the player to never switch up the bitrate during playback. We consider this parameter as a design choice for app developers. However, staying on a lower bitrate helps the player to maintain a lower latency lag compared to the static conditions. This statement also holds true for the other two profiles (S3-C0.1-L4 \& S4-C0.1-L5). From Fig. \ref{fig:comp_bsw} in general, we see a higher bitrate switch count in mobility scenarios compared to static. However, for the S4-C0.1-L5 profile, this is not true. We found that during driving sometimes the bitrate can quickly jump to a lower value because of extreme dynamic conditions (handovers, rapid drop in RSRQ). 
% This helps the player play the video with a stable latency lag and also results in a low bitrate switch count per run. 

Fig. \ref{fig:latency_rebuf_compare} shows the latency lag as a function of rebuffer event count for the three profiles. The dotted line represents the average latency lag for different scenarios. From the figure, we see that Latency Lag has a direct relation to the number of rebuffer events. Latency lag increases sharply with each rebuffering event. However, the average latency lag in some cases is lower in driving conditions compared to that of static and walking. For example, for the S2-C0.1-L3 profile, we noticed that during playback the bitrate 
switched to the lowest value within the first 3 minutes of playback and stayed on that which helped maintain a lower latency lag. This is again reflected in Fig. \ref{fig:comp_wb} where we see the lowest median weighted bitrate/min ($\sim$1 Mbps) compared to the other two scenarios. This is also true for the S3-C0.1-L4 profile. However, for the S4-C0.1-L5 profile, there is a noticeable increase in latency with respect to rebuffer events. The latency lag spikes to around 9 s with 4 rebuffer events counted during this run. This is again explained by Fig. \ref{fig:comp_wb}, where we see the average weighted bitrate for the driving run has some outliers (3.4 \& 4.5 Mbps) denoting the player switched bitrate slowly with each rebuffering event.

We conclude the following from our observations: (1) mobility in general hampers low-latency streaming. The weighted bitrate is lower compared to static conditions implying user-perceived QoE is worse during mobility, (2) due to dynamic conditions imposed by the mobility sometimes the player switches to the lowest bitrate rapidly which helps maintain a lower latency lag compared to static conditions, and (3) rebuffer events causes latency to increase rapidly implying that an efficient ABR algorithm must try to avoid stalls. 

\subsection{Correlation with Radio Signal Metrics} \label{RSRQ_find}
In this section, we expand our analysis to investigate the correlation of RAN side KPI with user QoE. Fig. \ref{fig:sample_driving_run} shows the timeline of one walking run and one driving run for the S4-C0.1-L5 profile. We plot the selected bitrate, latency lag, rebuffering events,  RSRQ, and Cell ID switch over time (20 mins). From the figure, we can see that the phone experiences a higher number of handovers (25 vs 2) and rebuffering events (4 vs 1) during driving compared to walking. We ignore the first and the last rebuffer events as they correspond to the playback start and end. We observe that RSRQ during driving varies significantly compared to walking and there is a strong correlation between RSRQ and rebuffer events. All the rebuffering events occur after a sharp drop in RSRQ (i.e., timestamp 16:07:52, 16:13:21). These rebuffer events also have an impact on the latency lag. Latency lag spikes after each rebuffer incident (timestamp 16:07:22,16:07:52,16:13:21). The sharp decrease in RSRQ also forces the player to drop its selected bitrate. However, by analyzing some walking runs we found that this is not always the case. This could also depend on the player's incorrect bandwidth estimation. We conjecture an overestimation misleads the player to remain on a higher bitrate, which would result in additional rebuffer events in the future.


 



